Katana: Dual Slicing-Based Context for Learning Bug Fixes

Contextual information plays a vital role for software developers when understanding and fixing a bug. Consequently, deep learning-based program repair techniques leverage context for bug fixes. However, existing techniques treat context in an arbitrary manner, by extracting code in close proximity of the buggy statement within the enclosing file, class, or method, without any analysis to find actual relations with the bug. To reduce noise, they use a predefined maximum limit on the number of tokens to be used as context. We present a program slicing-based approach, in which instead of arbitrarily including code as context, we analyze statements that have a control or data dependency on the buggy statement. We propose a novel concept called dual slicing, which leverages the context of both buggy and fixed versions of the code to capture relevant repair ingredients. We present our technique and tool called Katana, the first to apply slicing-based context for a program repair task. The results show Katana effectively preserves sufficient information for a model to choose contextual information while reducing noise. We compare against four recent state-of-the-art context-aware program repair techniques. Our results show Katana fixes between 1.5 to 3.7 times more bugs than existing techniques.

==> abstract.tex <==
\begin{abstract}

Contextual information plays a vital role for software developers when understanding and fixing a bug. Consequently, deep learning-based program repair techniques leverage context for bug fixes. However, existing techniques treat context in an arbitrary manner, by extracting code in close proximity of the buggy statement within the enclosing file, class, or method, without any analysis to find actual relations with the bug. To reduce noise, they use a predefined maximum limit on the number of tokens to be used as context. 
We present a program slicing-based approach, in which instead of arbitrarily including code as context, we analyze statements that have a control or data dependency on the buggy statement. We propose a novel concept called \emph{dual slicing}, which leverages the context of both buggy and fixed versions of the code to capture relevant repair ingredients. We present our technique and tool called \toolname, the first to apply slicing-based context for a program repair task. The results show \toolname effectively preserves sufficient information for a model to choose contextual information while reducing noise. We compare against four recent state-of-the-art context-aware program repair techniques. Our results show \toolname fixes between 1.5 to 3.7 times more bugs than existing techniques.

\end{abstract}

==> conclusion.tex <==
\section{Conclusion}
As a developer, context is pivotal while understanding and writing a fix for a buggy piece of code. Surrounding lines, methods, and class level information provide background contextual information that is important to devise a patch for a buggy piece of code. Current learning-based repair techniques adopt predefined heuristics, such as a limited number of tokens or AST nodes to extract context, which is insufficient for representing contextual information of a bug fix. We argue that context extraction needs to be directed toward relevant code for a learning-based repair technique to be effective. We present \toolname, the first technique to apply program slicing on a learning-based program repair task that includes relevant information as context pertaining to the buggy/fixed code. We show that program slicing through control and data flow analysis effectively preserves sufficient program repair ingredients %without introducing noise that can limit the model’s ability 
 to extract recurring patterns.  We propose the notion of \emph{dual slicing}, a novel approach that leverages context from both the buggy and corrected code. Our approach is able to fix 4,781 out of 11,397 bugs curated from open-source JavaScript projects. The results show that \toolname can resolve between 1.5 up to 3.7 times more bugs when compared to the state-of-the-art learning-based repair techniques. Furthermore, \toolname is effective across a wide range of bug patterns. % \toolname is scalable as it incorporates static information from source code and the overhead in processing time to extract slicing related information is minimal. 
 In the future, we plan to expand our interprocedural analysis, which is now limited to the enclosing file. We will also expand \toolname to support other programming languages such as Java. %We envision incorporating data and control flow edges to extract more semantic  information could be beneficial in improving the current techniques further.

==> discussion.tex <==
% !TEX root =  ../main.tex
\section{Discussion}

\change In this section, we discuss the findings from Section~\ref{sec:evaluation}.\stopchange{}

%Many studies have shown that noisy data can significantly impact the accuracy of a machine learning model \cite{noiseML}. From our experimental evaluation, we found that slicing helps to minimize noise and can retain relevant information to fix a buggy code instead of extracting context using ad-hoc heuristics as shown in Figure~\ref{fig:tokensdistro}.

\header{Role of slicing in learning repairs} The overall accuracy of \toolname in repairing programs can mainly be attributed to the effectiveness of dual slicing-based context. \change In Table~\ref{table:rq1}, we observe that dual slicing outperforms single slicing by a significant margin. Dual slicing can derive repair ingredients from both the buggy and fixed graphs. This additional contextual information allows the model to learn from buggy context and fixed context. For instance, the availability of vocabulary from the sliced context in fixed graphs during training equipped the model with repair ingredients needed for generating fixes during inference. We notice this in Listing~\ref{lst:dualfix}, where the fixed line replaces the variable \code{object} with \code{item} in which, the variable \code{item} is part of the vocabulary.

In addition to preserving the repair ingredients, program slicing can help to minimize noise for the GNN model.  \stopchange The quantitative analysis in Section \ref{slice-context-rq} shows the effect of program slicing in reducing the information scope, without the need for a predefined bound on the number of tokens or AST nodes. Listing~\ref{lst:slicefix} shows an example of a bug pattern that only \toolname could fix. The buggy file contains 550 lines of code. In the sequence-based approaches, although the variable \code{options} was present, the method \code{fetchVoiceRegions} was removed from the input due to their context limit. Even though the method was defined within the enclosing class and enclosing file, the low proximity between the method call and method definition caused this method definition to be truncated. While fixing a bug, the method signature provides useful debugging information to reason about the code. By leveraging slicing, \toolname was able to preserve relevant information pertaining to the buggy and fixed line. 
This indicates that dual slicing-based context can retain relevant information while reducing noise, which can benefit the learning process of the model, as shown in \autoref{table:rq3}.
%This indicates that dual-slicing based context can help preserve repair ingredients and minimize noise that could facilitate a learning-based model to generalize and generate a fix.

\vspace{0.5em}
\begin{lstlisting}[backgroundcolor=\color{white},frame=1,label={lst:cbpatch},frame=single,framesep=5pt,backgroundcolor=\color{lightgray},
	rulecolor=\color{lightgray}, numbers=none,label={lst:slicefix},caption={Example of a bug fixed by \toolname}]
-   this.fetchVoiceRegions(options);
+   this.fetchVoiceRegions();
\end{lstlisting}
\vspace{0.5em}

\begin{landscape}
\begin{table}[!h]
	\scriptsize
	\centering
	\caption{Qualitative analysis of bugs fixed exclusively by \toolname.}
	{
		\begin{tabular}{p{2.6cm}p{3.2cm}p{5.2cm}p{5.2cm}}
			\toprule
			\textbf{Bug Pattern} & \textbf{Description} & \textbf{Buggy Code} & \textbf{Fixed Code} \\
			\midrule
			Same Function More Args & \emph{Function with missing argument in the buggy line} & \lstinline|return drones[droneUpdate.id] = new Drone(droneUpdate);| & \lstinline|return drones[droneUpdate.id] = new Drone(droneUpdate, 10);| \\
			\cmidrule[0.3pt]{3-4}
			
			&  & \lstinline|currentUser: service();| & \lstinline|currentUser: service(user);|  \\
			\cmidrule[0.4pt]{1-4}
			
			Same Function Less Args & \emph{Function with additional argument in the buggy line} & \lstinline|kittens.pop(name)| & \lstinline|kittens.pop()|  \\
			\cmidrule[0.3pt]{3-4}
			
			&  & \lstinline|app.get('/api/current_user', (req, res, next) => { | & \lstinline|app.get('/api/current_user', (req, res) => { |  \\
			\cmidrule[0.4pt]{1-4}
			
			Incorrect Object Instantiation & \emph{Constructor invoked without} \lstinline|new| \emph{keyword} & \lstinline|var componentSchema = Schema({ | & \lstinline|var componentSchema = new Schema({ |  \\
			\cmidrule[0.3pt]{3-4}
			
			&  & \lstinline|const history = mongoose.Schema({ | & \lstinline|const history = new mongoose.Schema({ |  \\
			\cmidrule[0.4pt]{1-4}
			
			Missing Return Statement & \emph{Expression with missing} \lstinline|return| \emph{keyword} & \lstinline|await bcrypt.compare(password, savedPassword);| & \lstinline|return await bcrypt.compare(password, savedPassword);|  \\
			\cmidrule[0.3pt]{3-4}
			
			& & \lstinline|changeAnimal();| & \lstinline|return changeAnimal();|  \\
			\cmidrule[0.4pt]{1-4}
			
			Incorrect Variable Declaration & \emph{Variable declared with incorrect keyword} & \lstinline|var shuffled = arr.slice(0), i = arr.length, min = i - count, temp, index;| & \lstinline|let shuffled = arr.slice(0), i = arr.length, min = i - count, temp, index;|  \\
			\cmidrule[0.3pt]{3-4}
			
			&  & \lstinline|var garray = array//.shift()| & \lstinline|const garray = array//.shift()|  \\
			
			\cmidrule[0.4pt]{1-4}
			
			Incorrect For Loop Used & \emph{Expression with incorrect usage of} \lstinline|for...in| \emph{or}  \lstinline|for...of| \emph{used} & \lstinline|for (var file in files) {| & \lstinline|for (var file of files) {| \\
					\cmidrule[0.3pt]{3-4}			 
					
					&  & \lstinline|for (let slot of Object.values(character.slots)) {| & \lstinline|for (let slot in Object.values(character.slots)) {| \\
			\cmidrule[0.4pt]{1-4}
			
			Change Boolean Literal & \emph{Expression with incorrect boolean literal used} & \lstinline|app.use(bodyParser.urlencoded({ extended: false }));| & \lstinline|app.use(bodyParser.urlencoded({ extended: true }));|  \\
			\cmidrule[0.3pt]{3-4}
			
			&  & \lstinline|overlap: {type: Boolean, default: true},| & \lstinline|overlap: {type: Boolean, default: false},|  \\
			\cmidrule[0.4pt]{1-4}
			
			Change String/Numeric Literal & \emph{Expression with incorrect string/numeric literal used} & \lstinline!const PORT = process.env.PORT || 3001;! & \lstinline!const PORT = process.env.PORT || 3000;!  \\
			\cmidrule[0.3pt]{3-4}
			
			&  & \lstinline|router.get('/comment/:id', CommentController.GetComments);| & \lstinline|router.get('/comment/list', CommentController.GetComments);| \\
			\cmidrule[0.4pt]{1-4}
			
			Change Identifier Used & \emph{Expression with incorrect identifier used} & \lstinline|componentWillMount: () => {| & \lstinline|componentDidMount: () => {| \\
			\cmidrule[0.3pt]{3-4}			 
			
			&  & \lstinline|this.destroy(res, res)| & \lstinline|this.destroy(res, err)| \\
			
			\bottomrule
		\end{tabular}
	}
	\label{table:patch_analysis}
\end{table}
\end{landscape}

\header{\toolname is effective across pervasive bug patterns} Table \ref{table:patch_analysis} shows a qualitative analysis of the type and description of bug patterns observed in the test dataset that only \toolname was able to fix. \change Unlike prior techniques~\cite{pradeloopsla, li:suspicious-return-stmnt:20, scott:detecting-swapped-arguments:20} which are trained on specific error types, our model targets a wide variety of error types as it is trained on real world bugs.\stopchange{} We assessed 100 random samples out of the 891 correct patches generated uniquely by  \toolname (see Figure \ref{fig:venn}, second column from right). As mentioned previously, our dataset has been curated from open-source Github repositories and hence, they are representative of real bugs that have been fixed by developers. For the qualitative analysis of the patches, the authors manually analyzed the resulting correct patches of \toolname, categorized them individually and came to a consensus if they agreed on the bug fixes to be representative of bug patterns. The assessment of the patches and categorization took approximately 12 person-hours in total.
For labelling the bug type, we used ManySStuBs4J~\cite{minesstubs} to identify the category of the bug fixes. We present nine bug patterns (two patches per pattern as examples) fixed by \toolname in Table \ref{table:patch_analysis}  in the test dataset. Among these nine bug patterns, five represent some common single statement bugs seen in other programming languages such as Java or Python~\cite{minesstubs,PySStuBs}. The remaining four patterns are specific to JavaScript. %these bugs would have been detected early on by Java compilers. 
These language-specific bug patterns include  \emph{Incorrect Object Instantiation}, \emph{Missing Return Statement}, \emph{Incorrect Variable Declaration} and \emph{Incorrect For Loop Used}. Since JavaScript code is interpreted at runtime, bugs such as \emph{Incorrect Object Instantiation} and \emph{Missing Return Statement} may only surface during program execution. %or , not surface at all. 
These bugs occur because JavaScript is a dynamically typed language and can silently propagate these errors. \emph{Missing Return Statement} has been categorized as a common bug pattern in JavaScript in BugsJS~\cite{bugsjs}. \emph{Incorrect Variable Instantiation} is a common best practice in modern JavaScript projects that supports the ECMAScript 6 (ES6) syntax, and it indicates a code smell. In ES6, the keywords \code{let} and \code{const} were introduced to the language \cite{es6} because of scoping issues caused by the keyword \code{var}, which can eventually lead to hard to find bugs in JavaScript~\cite{jsScoping}. Another bug type, \emph{Incorrect For Loop Used}, occurs mainly in ES6 compatible JavaScript source code, where the \code{for...in}  and \code{for...of} loops are incorrectly used in which the former is used for looping through enumerables in objects and the latter is used for iterating through values of arrays and objects. Due to their syntactical similarity, developers often tend to use them interchangeably for the wrong purpose which can lead to bugs that are hard to identify. Thus, \toolname can detect and fix a wide variety of pervasive bug patterns that include both common and language-specific bugs more effectively than the baselines. 

\iffalse
\header{Scalability and execution} \toolname uses static analysis to generate slices with respect to the buggy and fixed lines. %Unlike dynamic slicing which relies on execution of the program to generate the relevant statements, static slicing outputs all possible statements with respect to the slicing criterion. This approach is therefore, less costly because it can help in generating a patch without relying on the executed output of a program.
%
%Contrary to traditional program repair tools which rely on a set of rules to repair each type of bug patterns, our slice based program repair approach is data-driven. By analyzing real bugs from open source commits fixed by developers, \toolname was able to fix common bug patterns by solely relying on the training set. The main advantage of learning based repair techniques is that it does not require domain knowledge to add a new bug pattern for generating fixes. In this way, \toolname is scalable in fixing a wide variety of real bugs with no additional cost to a developer.
%
In terms of analysis time, it takes around 0.49 seconds to perform dual slicing for a single datapoint (pair of buggy and fixed files). It took around 16 hours to generate the sliced version of the whole dataset. The training of the model took 1.7 hours and inference took 1.5 hours for beam size 3. 

% whereas training unsliced code in \hoppity with 500 nodes limit took 2.5 hours. Using a beam size of 3, our approach is 2 times faster during inference as it takes 1.5 hours to generate 3 candidate patches, whereas for \hoppity, it takes around 3.05 hours.
\fi

\iffalse
\begin{lstlisting}[backgroundcolor=\color{white},frame=1,label={lst:cbpatch},frame=single,
	framesep=3pt,basicstyle=\small\ttfamily,
	rulecolor=\color{darkgray}, numbers=none,caption={Example of \emph{Same function less args} patch inside a callback.}]
-   client.on("ready", (channel) => {
+   client.on("ready", () => {
\end{lstlisting}
\fi

\header{Effect of missing repair ingredients on inference} \toolname is most effective when it can incorporate relevant repair ingredients by leveraging context using slicing. To understand why \toolname was unable to correctly generate patches for some bugs, we manually examined 200 random samples from the incorrect patches. Upon careful investigation, we observed that for 16\% of the incorrect patches,  the relevant repair ingredients were not present within the file. Since we collect our datapoints based on buggy commits, our scope is limited to the enclosing file, which often does not include  interdependent files. As such, we found instances of function calls or variables used in the buggy file that were imported from other files.  As a result, relevant syntactic and semantic information required for such functions or variables was not preserved as context for the model to generate correct patches. To mitigate this, we plan to extend our slicing technique to perform interprocedural analysis \emph{across files} as part of future work.

Furthermore, there were recurring instances (84\%) of the \emph{Change String/Numeric Literal} bug pattern among the incorrect patches generated by \toolname. Upon closer inspection, we noticed that not all of these string replacements were actual bug fixes---most of them were typo fixes or ad-hoc textual changes in config files. We believe that bug patterns pertaining to string changes can further benefit from a larger vocabulary size than the current 5,002 tokens.

%Furthermore, we plan to incorporate copy mechanism in the model to handle the unknown vocabulary problem.

%However, as shown in Figure~\ref{fig:venn}, \toolname was not able to fix 420 instances of bugs that Tufano et al.~\cite{tufano:tosem:19} alone would fix, or the 148 bugs that \hoppity alone could fix. 

%As Tufano et al.~\cite{tufano:tosem:19} employ abstraction for non-frequent tokens to limit the vocabulary size, the search space during beam search decoding is significantly narrower in comparison to \toolname. %the probability of correct patch generation for such bug patterns is higher.
%Tufano et al.~\cite{tufano:tosem:19} used a vocabulary size of 815 containing abstracted tokens whereas \toolname used a 6.14 times larger vocabulary with 5,002 tokens. We believe that bug patterns pertaining to string changes can benefit from adopting copy mechanism in the model, which we aim to explore in the future.

%We believe that bug patterns pertaining to string changes can further benefit from abstractions in the source code representation, which we aim to explore in the future.

\iffalse
In case of \hoppity, we noted that it was able to fix 148 bugs uniquely, compared to other approaches (last column in Figure~\ref{fig:venn}). \hoppity filters out datapoints larger than 500 nodes for optimal performance, however, we have kept our vocabulary size the same and added a variety of graph sizes based on the sliced context. Hence, we hypothesize that having more number of large graph samples can help learn recurring patterns of larger graph sizes. 
\fi

\header{Limitations} \toolname cannot currently generate slices from minified or obfuscated JavaScript code because of constraints in our slicing framework. The minification step removes whitespaces, obfuscates variable names and often produces a single line as an output. In practice, the minification step is taken prior to deployment in the production environment, and it is not for human consumption. Therefore, we excluded minified JavaScript files in our dataset as they may introduce noise in the learning process. 

\change Some JavaScript files can contain templated code (i.e., HTML or JSX\footnote{https://reactjs.org/docs/introducing-jsx.html}) from front-end frameworks such as ReactJS\footnote{https://reactjs.org}, VueJS\footnote{https://vuejs.org} or Angular\footnote{https://angular.io}. However, our analysis tool cannot extract slices for bugs inside front-end templated code. Consequently, \toolname could produce invalid code slices because the files do not contain pure JavaScript code. \stopchange{}

\change JavaScript is a dynamically typed language, which inherently makes it difficult to keep track of control and data flow dependencies during program slicing. In cases where control and data flow analysis does not yield any sliced context, we consider the contents of entire file as context scope for the buggy line. \stopchange{}

% bugs that \hoppity was able to fix 420 bugs that only Tufano et al.~\cite{tufano:tosem:19} could fix.  In an attempt to explain why \toolname was unable to fix certain bugs, we qualitatively assessed a subset of the patches generated by \hoppity and Tufano et al. Almost all of the patches fixed by only unsliced code were bug patterns of type \emph{Change String Literal} and \emph{Same Function Less Args}. Only 8 of the patches were related to the bug pattern \emph{Same Function Less Args} and the rest were string replacements. However, not all of the string replacements were bug fixes - most of them were simply typo fixes or just text changes in config files. We believe that \hoppity with unsliced contextual data was correctly able to predict these fixes because of the consistent number of graph sizes used in their data. \hoppity filters out datapoints larger than 500 nodes, nevertheless, we have kept our vocabulary size the same and added a variety of graph sizes based on the sliced context. Hence, we hypothesize that more large graph samples can help learn recurring patterns of larger graph sizes.


==> evaluation.tex <==
% !TEX root =  ../main.tex
\section{Evaluation}
\label{sec:evaluation}

To assess the effectiveness of \toolname we address the following research questions: 

\newlist{researchquestions}{enumerate}{1}
\setlist[researchquestions]{label*=\textbf{RQ\arabic*}}

\begin{researchquestions}
	
	\item How does dual slicing compare to single slicing for learning repairs? 

	%\item What is the effect of slicing-based context on the amount of information?	
	%\item What is the role of  slicing-based context to preserve repair ingredients?
	
	\item How does \toolname compare to state-of-the-art learning-based repair techniques?
	   
	\item What is the effect of slicing on the information obtained as context? 
   
    %\item How does context window affect program repair accuracy in \toolname?    
\end{researchquestions} 

We discuss the experiments that we designed to answer each of the research questions in the following subsections and outline the results.

%\subsection{Effect of slicing-based context to preserve repair ingredients (RQ1)}


\subsection{Single versus dual slicing as context (RQ1)}
We compare the effectiveness of single slicing where we extract context from the buggy file with dual slicing where the context is extracted from both the buggy and fixed files. 

Using our initial 91,181 (training) datapoints, we generated two separate datasets using our single and dual slicing techniques. The processing time to generate slicing is negligible. On average, single slicing and dual-slicing analysis takes around 330 and 490 milliseconds for a single datapoint, respectively. With the tuned set of hyperparameters, we trained two models separately with the generated single sliced and dual sliced datasets. It took 1.7 hours to train each model for 50 epochs. The average inference time for a datapoint is around 2.54 seconds for each trained model. All our experimental runs are performed on an Ubuntu Linux 18.04.2 LTS server with 122 GB RAM, 16 vCPUs and 2,000 GB SSD. 

\begin{table}%[th]
	\small
	\centering
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\caption{Accuracy of single slicing vs. dual slicing}
	{
		\begin{tabular}{l | rrr}
			\toprule
			\multirow{2}{*}{\textbf{Approach}} 	& \multicolumn{3}{c}{\textbf{Accuracy}} \\
			\cmidrule[0.3pt]{2-4}
			& \textbf{Top-1}    & \textbf{Top-3 }  & \textbf{Top-5}   \\
			\cmidrule[0.3pt]{1-4}
			Single Slicing	& 20.72\% &  35.01\% & 42.90\%  \\
			Dual Slicing & 28.31\% & 41.95\%  & 46.96\%  \\
			\bottomrule
		\end{tabular}
	}
	\label{table:rq1}
\end{table}

We use the same test dataset to evaluate the accuracy of the two models. As the model produces a series of graph edits to generate the patch, we consider an output to be correct if the predicted location of the AST node, the type of operation (i.e., replace type or value, add node, delete node) and the value of the node matches the expected node location, operation type, and value of the patch in the test dataset, for the entire sequence of graph edits. 

Table \ref{table:rq1} shows the results for single and dual slicing in \toolname. 
Single sliced context yielded accuracies of 20.72\%, 35.01\%, and 42.90\% with beam sizes of one, three, and five, respectively. 
Dual sliced context yielded accuracies of 28.31\%, 41.95\%, and 46.96\%, respectively.  Dual slicing achieved higher accuracies for all beam sizes, with 37, 20, and 9 percent increases for the top-1, top-3, and top-5 suggestions, respectively, with respect to single slicing. 
%Figure \ref{fig:venn} shows the overlap of correct predictions using beam size 3 generated by the two types of slicing approaches. 

For instance, if we focus on top-3 suggestions, out of the 11,397 bugs in the test dataset, dual slicing fixed 4,781 and single slicing fixed 3,990. Out of these, 3,984 were fixed by both single and dual slicing, however, the dual slicing approach was able to fix 797 more bugs than single slicing.
% and six were fixed only by single slicing. 

%To understand why dual slicing was unable to fix those that were fixed by single slicing, we analyzed the six bugs. Four of the bug fixes were of type \emph{Change String Literal} and two of the bug fixes were of type \emph{Same Function Less Args}. The context for both single and dual slicing were the same for string literal changes, however for the type \emph{Same Function Less Args}, the removal of the variable in the fixed line also removes the context of that removed variable in the dual sliced fixed file. Although dual slicing could fix these bugs patterns in most cases, we believe that larger number of recurring patterns can help dual slicing in fixing these bugs more effectively.

%Due to this, dual sliced context in the buggy line was producing no context in the fixed file, whereas single sliced context added the same context surrounding the buggy line into the fixed file. In order to find a pattern in the bug fixing capability of dual sliced context, we analyzed 10 random samples from the 797 bugs that only dual slicing predicted correctly. Out of the 10 correct predictions, we verified 3 samples having the bug pattern \emph{Change Identifier Used}. We attribute this pattern to the availability of repair ingredients due to dual slicing. Listing~\ref{lst:dualfix} demonstrates an example of such a bug that we identified through random sampling (in addition to our running example in Listing~\ref{lst:mot1}).

\vspace{0.5em}
\begin{lstlisting}[backgroundcolor=\color{white},frame=1,label={lst:cbpatch},frame=single,
framesep=5pt,backgroundcolor=\color{lightgray},
rulecolor=\color{lightgray}, numbers=none,label={lst:dualfix},caption={Example of \emph{Change Identifier Used} bug pattern fixed by dual slicing}]
-   cart.push(object);
+   cart.push(item);
\end{lstlisting}
\vspace{0.5em}

Listing \ref{lst:dualfix} shows an example of a bug that was correctly fixed by dual slicing but was not repaired by single slicing. Through sampling, we verified that \emph{Change Identifier Used} is one of the recurring patterns among the correct patches generated by dual slicing. We attribute this pattern to the availability of repair ingredients, made accessible through dual slicing as context used during training. Therefore, since the dual sliced context outperforms the single sliced context, we select it as our default approach in \toolname going forward.

\subsection{Comparison with state-of-the-art (RQ2)}

We compare \toolname with the four recent deep learning-based program repair techniques. \change In addition, we considered evaluating DLFix~\cite{dlfix}. However, DLFix was unavailable at the time of writing this paper. A brief outline of these state-of-the-art deep learning-based program repair techniques is described below\stopchange{}:

\begin{enumerate}	
	\item \textbf{Tufano et al. \cite{tufano:tosem:19}} employs code abstraction on an RNN-based NMT model with attention mechanism.
	\item \textbf{\sequencer \cite{sequencer}} uses an RNN-based NMT model equipped with copy mechanism.
	\item \textbf{\hoppity \cite{hoppity}} proposes a GNN model to predict the location of bug and generate a fix through a sequence of graph edits.
	\item \textbf{\coconut \cite{coconut}} leverages a CNN-based NMT model with two separate encoders for buggy line and context.
\end{enumerate}

%, uses a TreeRNN based architecture that represents source code as a tree. We were unable to evaluate DLFix since the artefacts for DLFix were unavailable when writing this paper. However, a more recent work, \coconut, used numbers reported by DLFix on the Defects4J dataset and demonstrated superior performance.

\subsubsection{Characterizing context}
To characterize how current techniques treat context, we reason about five different aspects of context:

\begin{itemize}
\item \textbf{Analysis}: Contextual information can be extracted from the source code in various ways. The analysis can be as simple as naively extracting tokens from the buggy statement's surroundings, to more complex program analysis techniques such as data flow, control flow, or slicing. 

\item \textbf{Representation}: Once extracted, context can be represented in different ways, e.g., as linear sequence of tokens, or nodes in a graph.

\item \textbf{Scope}: Different levels of granularity can be considered for the scope of context, for example, by focusing on the entire program, enclosing file, class, or method. 

\item  \textbf{Proximity}: Context can be extracted with respect to the location of the bug/fix, e.g., surrounding, before, or after the buggy line.

\item \textbf{Limit}: Context size can be limited by the amount of information it contains, e.g., number of lines of code, tokens, or AST nodes. 

\end{itemize}

\begin{table}[ht]
	\scriptsize
	\centering
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\caption{Accuracy comparison of \toolname with other learning-based program repair techniques.}
	%evaluated on 11,397 bugs from test set. The approaches are trained on the same dataset of 91,181 real JavaScript bugs.
	\resizebox{\textwidth}{!}		
	{
		\begin{tabular}{l | lllll | rrr}
			\toprule
			\multirow{2}{*}{\textbf{Approach}} 	& \multicolumn{5}{c|}{\textbf{Context}}	& \multicolumn{3}{c}{\textbf{Accuracy}} \\
			\cmidrule[0.3pt]{2-9}
			& \textbf{Analysis} & \textbf{Representation} & \textbf{Scope} & \textbf{Proximity} & \textbf{Limit} 						& \textbf{Top-1}    & \textbf{Top-3 }  & \textbf{Top-5}   \\
			\cmidrule[0.3pt]{1-9}
			Tufano et al.~\cite{tufano:tosem:19}		 		& Naive 					& Sequences of tokens		& 	Enclosing method 					& Before/After				 	&	100 tokens 			& 4.90\% 					& 11.33\% & 15.84\%  \\
			\sequencer~\cite{sequencer} 				& Naive						& Sequences of tokens		&  Enclosing class  & Before/After					&  1000 tokens 			&7.99\% 					& 13.84\% & 18.08\%  \\
			\hoppity~\cite{hoppity} 					& Naive						& AST-based graph						&  Enclosing file  						& Before/After					&  500 nodes	 		& 5.05\% & 14.40\% & 19.62\% \\
			\coconut~~\cite{coconut}  					& Naive						& Sequences of tokens		&	Enclosing method 					&	Before/After					& 1,022 tokens 			& 24.67\% & 27.90\% & 28.97\% \\			
			\textbf{\toolname} 	& \textbf{Dual Slice} 			& \textbf{AST-based graph} 					&  \textbf{Enclosing file}  						& 	\textbf{Before}							&	\textbf{N/A}					&	\textbf{28.31\%} &\textbf{41.95\%}  & \textbf{46.96\%}  \\
			\bottomrule
		\end{tabular}
	}
	\label{table:rq3}
\end{table}


Table~\ref{table:rq3} compares how state-of-the-art techniques treat context using these five aspects. 

\subsubsection{Setup} %Except for \hoppity, each of these state-of-the-art learning-based approaches has been trained on Java source code corpus as their dataset. Therefore, in order to have a fair comparison, 
We trained a separate model using the deep learning framework of each of these techniques following the dataset split of Table~\ref{table:data_split} with our unsliced dataset as follows:

Tufano et al. \cite{tufano:tosem:19} represent source code as a sequence of tokens and use the method enclosing the bug as the scope of context, which is limited by a maximum of 100 tokens. There is no program analysis for extracting context. However, abstraction is applied to code to limit the vocabulary size. We applied the same abstraction technique to our JavaScript dataset. We tokenized the buggy and fixed JavaScript files and tokenized it using js-tokens\footnote{https://www.npmjs.com/package/js-tokens} to discern whether a given token is an identifier, method, or a literal. Following the same approach as ~\cite{tufano:tosem:19}, we maintain a dictionary of frequently occurring tokens and replace the remaining tokens with abstraction depending on the token type (e.g.,  METHOD\_1, VARIABLE\_1). Additional challenges with JavaScript code included the presence of JSX identifiers and literals. We assigned new abstractions for these types of tokens. The final vocabulary size became 815, including abstractions, JavaScript keywords, and frequent tokens. %We then trained a seq2seq model with our preprocessed dataset.

\sequencer represents source code as a sequence of tokens. However, they use the enclosing class as context scope, limited by  1,000 tokens; it delineates the buggy line within <START\_BUG> and <END\_BUG> tokens for differentiation within the context. \sequencer takes more input tokens from lines that appear before the buggy line. It extracts 2/3rd more tokens from proceeding statements before the buggy line than the subsequent statements. We applied the same technique to our JavaScript code corpus, and if the buggy line was not encapsulated in a class, we extracted tokens from the surrounding lines in the JavaScript file. The vocabulary size is limited to 1,000 tokens. %After pre-processing, we used their NMT model with copy mechanism for training and inference.

\hoppity represents context as an AST-based graph and does not apply any program analysis. Its context scope is the enclosing file of the buggy line, limited to 500 AST nodes. The vocabulary size on our dataset is 5,003 tokens.

\coconut leverages the enclosed method of the buggy line as the scope of context and represents the source code as a sequence of tokens limited by 1,022 tokens. Similar to other techniques, context is taken without any program analysis. They employ abstraction and use two separate encoders to feed the buggy line and context. We used pre-processing scripts from their artefact to tokenize source code, and the resulting vocabulary size was 63,499. %Following their technique, we employed the CNN-based encoder-decoder NMT model. 

We use the same test dataset of 11,397 JavaScript bugs for evaluating all the models. The best reported hyperparameter settings and epochs were used to train each of these models. To keep the accuracy comparison equitable across all the models, we use beam sizes of one, three, and five. 

\subsubsection{Results} 
Table  \ref{table:rq3} reports the obtained accuracies for beam sizes of one, three, and five in the columns \emph{Top-1}, \emph{Top-3} and \emph{Top-5}. The lowest \emph{Top-1} accuracy was yielded by Tufano et al.~\cite{tufano:tosem:19}. Despite using a high level of abstraction and a small vocabulary size, limited contextual information has not helped their model. As more contextual information was fed into the model, accuracy improved gradually. \hoppity demonstrated better accuracy for \emph{Top-3} and \emph{Top-5} predictions. Among existing techniques, \coconut yielded the highest accuracy. However, \toolname outperforms all existing techniques for all the beam sizes, with accuracies of 28.31\% , 41.95\%, and 46.96\%  for the beam width 1, 3, and 5, respectively. %The beam size of 1 yields the lowest accuracy, and the increase in accuracy from beam 3 to 5 five is smaller than the jump from beam 1 to 3. 

Considering the top-3, \toolname is 270.26\%, 203.11\%, 191.32\%, 50.36\% more accurate in fixing buggy programs than Tufano et al.~\cite{tufano:tosem:19}, \sequencer, \hoppity, and \coconut, respectively. By learning from the context of the relevant statements in the buggy and fixed file, the dual slicing-based context in \toolname can accurately repair buggy programs by a significant margin.
%Considering the top-3, \toolname is  3.7, 3.0, 2.9, and 1.5 times more accurate in fixing buggy programs than Tufano et al.~\cite{tufano:tosem:19}, \sequencer, \hoppity, and \coconut, respectively. By learning from the context of the relevant statements in the buggy and fixed file, the dual slicing-based context in \toolname can accurately repair buggy programs by a significant margin.

Figure \ref{fig:venn} demonstrates an illustration of the overlapping sets of top-3 correct patches generated by the repair techniques. Each row in this figure represents a specific approach which is color encoded for differentiability. The numbers on the right depict the total number of patches generated correctly by each approach. For example, \toolname can fix a total of 4,781 out of 11,397 bugs, \coconut can fix 3,180 out of 11,397 bugs correctly and so on. The numbers at the bottom indicate the intersecting set of the correct patches for the specific block. For example, 888 patches of the same set of bugs were correctly generated by \toolname, \coconut, and \sequencer, as shown at the bottom. As three approaches overlap, this number is reflected at the top row in this column of 888 patches. All five techniques could accurately fix 101 instances of bugs as indicated by the presence of all colors in the leftmost first column in Figure~\ref{fig:venn}. We observe that \toolname can fix a wide range of bugs, and the row for \toolname encompasses patches from other approaches. Furthermore, 891 bugs could only be fixed by \toolname as shown in the figure.

\begin{figure}%[ht]
	\centering
	\includegraphics[width=244pt]{images/supervenn2.pdf}
	\caption{Overlap of top-3 correct patches generated by context-aware learning based approaches.}
	\label{fig:venn}
\end{figure}


%\toolname was able to fix 3,930, 3,266, 3,288 and 1,605 more bugs than the baselines Tufano et al.~\cite{tufano:tosem:19}, \sequencer, \hoppity and \coconut, respectively. \ali{why am I not seeing any of these numbers on the figure? }

\subsection{Slicing-based context (RQ3)}
\label{slice-context-rq}
%For RQ1, we examine the implications of using program slicing as context to retain the necessary information for generating a fix in comparison to other context-aware learning-based program repair techniques. 
We carry out a quantitative analysis of our slicing technique to measure the type and amount of information considered as context and compare it against other approaches. 


We collected statistics over our dataset during the program slicing analysis. We calculated the number of lines before and after slicing as well as the fraction of the datapoints undergoing control flow and data flow analysis. We found that 26.96\% of the total datapoints (113,975 pairs of buggy and fixed files) required the use of both control flow and data flow analysis to produce the slices. The remaining 73.04\% were sliced by data flow analysis only. Figure \ref{fig:boxplot} illustrates the number of lines before and after slicing across the datapoints. Here, we refer to the dataset before slicing as unsliced. 

\begin{figure}[h]
	\centering
	\includegraphics[width=150pt]{images/sliced-unsliced-lines-beanplot.pdf}
	\caption{Distribution of number of lines in Sliced and Unsliced data.}
	\label{fig:boxplot}
\end{figure}


\toolname's program slicing reduced the average number of lines to consider for context  from 39 to 15. The median number is also reduced from 33 to 9. The maximum number of lines before slicing is 1,087, and after slicing it is reduced to 636, whereas the minimum is 1 in both cases.

\begin{figure}[t]
	\centering
	\includegraphics[width=150pt]{images/linechart.pdf}
	\caption{Reduction in number of lines after slicing across datapoints.}
	\label{fig:linediff}
\end{figure}

 In Figure \ref{fig:linediff}, we can observe the spread of line differences across the datapoints. The difference from sliced to unsliced is always positive indicating reduction after slicing. The average reduction is 24 lines. The maximum reduction is 1,073 lines, for a file that was 1,087 lines. %; this corresponds to the maximum in the unsliced dataset as seen in Figure \ref{fig:boxplot}.




\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.14\textwidth}
		\centering
		\includegraphics[width=\textwidth,height=150pt]{images/tufano.pdf}
		%\caption{Tufano}
		\label{fig:tufanotokens}
	\end{subfigure}
%	\hfill
	\begin{subfigure}[b]{0.14\textwidth}
		\centering
		\includegraphics[width=\textwidth,height=150pt]{images/sequencer.pdf}
		%\caption{SequenceR}
		\label{fig:sequencertokens}
	\end{subfigure}
%	\hfill
	\begin{subfigure}[b]{0.14\textwidth}
		\centering
		\includegraphics[width=\textwidth,height=150pt]{images/hoppity.pdf}
		%\caption{Hoppity}
		\label{fig:hoppitytokens}
	\end{subfigure}
%	\hfill
	\begin{subfigure}[b]{0.14\textwidth}
		\centering
		\includegraphics[width=\textwidth,height=150pt]{images/coconut.pdf}
		%\caption{Coconut}
		\label{fig:coconuttokens}
	\end{subfigure}
%	\hfill
%	\hfill
	\begin{subfigure}[b]{0.14\textwidth}
		\centering
		\includegraphics[width=\textwidth,height=150pt]{images/katana.pdf}
		%\caption{Katana}
		\label{fig:katanatokens}
	\end{subfigure}
%	\hfill
	\caption{Descriptive statistics of tokens in context-aware learning approaches.}
	\label{fig:tokensdistro}
\end{figure*}

Figure \ref{fig:tokensdistro} depicts bean plots of the number of tokens in the buggy files for \toolname and the other techniques. We chose the buggy files from our (113,975)  JavaScript datapoints because the machine learning model takes the buggy file or buggy line with context as the input during inference. We stripped the whitespaces and comments from these files before token analysis. Tokens are the smallest possible unit that is common between all these approaches. Hence, we examine the increase or reduction of information used as context through this metric. As discussed before, except for \toolname, all of these context-based approaches use an ad-hoc bounding limit for reducing noise in the context. Just to recap, \hoppity uses a maximum limit of 500 nodes whereas \sequencer, Tufano et al. and \coconut use a sequence limit of 1,000, 100 and 1,022 tokens, respectively. Among all the approaches, \hoppity has the highest maximum token count of 3,589 tokens followed by \coconut (1,019 tokens), \sequencer (1,000 tokens) and Tufano et al. (100 tokens). The maximum number of tokens in \toolname is 2,399 tokens. Our slicing reduced the number of tokens by 1.5 times compared to \hoppity. \hoppity has the highest average number of 290 tokens, and with abstraction, Tufano et al. have the lowest average of 80 tokens. The average number of tokens in \sequencer and \coconut are 209 and 190, respectively. \toolname has an average of 132 tokens, which is less than \hoppity, \sequencer and \coconut. The median number of tokens shows a more profound effect of program slicing in the reduction of tokens. \toolname has the lowest median of 84 tokens among all the approaches. We can also observe the same trend of token reduction in the lower quartile of the dataset with \toolname. For the third quartile of the dataset, \hoppity, \sequencer and \coconut have 411, 301, and 269 tokens, respectively. On the other hand, Tufano et al. and \toolname yielded 68 and 160 tokens, which is significantly lower. Without a need for truncating the context, our approach for extracting relevant context based on control and data flow analysis, has a significant amount of information reduction on average.



\iffalse
\subsection{RQ4: How does context window affect program repair accuracy in \toolname?}

\toolname in dual sliced mode is able to predict the patch for buggy JavaScript program with an accuracy of 41.95\% without any limit to the maximum number of nodes in the graphs. However, we want to verify whether limiting the number of nodes would further increase the model's accuracy in predicting a fix. We conduct an empirical analysis and compare the effect of context window on both \toolname and the baseline. To this end, we trained a total of 8 additional models in both \toolname and \hoppity with varied number of maximum nodes. This means that datapoints more than the maximum number of nodes will not be considered in training or testing in the model. We chose 5 categories of maximum nodes to assess the effect of context window. The reason for selecting 315 and 1,600 nodes is because it represents an approximation of the 25th and 99th percentile of the number of nodes found in unsliced dataset. 500 nodes is chosen because it the default maximum number of nodes in \hoppity \cite{hoppity} and 1,000 nodes is chosen as a midpoint between 500 and 1,600. Figure \ref{fig:ctx_window} illustrates the effect of graph node limit on the patch prediction accuracy of \toolname and against the baseline.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{images/ctx_window.pdf}
	\caption{Effect of context window on Accuracy.}
	\label{fig:ctx_window}
\end{figure}

In Figure 7, we can see that as the number of node increases, the accuracy of program repair decreases gradually. The highest accuracy for both sliced and unsliced data at 315 nodes is 42.75\% and 16.08\% respectively. The lowest accuracy for dual sliced and unsliced is 40.65\% and 9.82\% respectively when the maximum number of nodes is 1,600. However, when there is no limit to the number of nodes, the accuracy slightly increases (41.95\% for dual sliced and 10.78\% for unsliced) when compared to a limit of 1,600 nodes. We believe that this small improvement in accuracy can be due to the inclusion of slightly more data, as certain datapoints have not been excluded due to the max nodes limit. We can also observe that the effect of context window in accuracy is greater for unsliced dataset rather than dual sliced dataset. This further strengthens the effectiveness of dual slicing based context over unsliced. We believe that, dual sliced dataset is already sufficient enough in delivering meaningful context for a learning model to predict fixes and reducing noise, which is why the effect of reducing context window is negligible compared to the unsliced data. 
\fi

==> introduction.tex <==
% !TEX root =  ../main.tex
\section{Introduction}

% What the intro should say:
  % Program repair 
  % Learning-based PR
  % Context in LBPR (others)
  % Katana (novelty)
  % Contributions

Traditional automated error detection~\cite{google:sa} and program repair~\cite{legouesNFWTSE2012,Scott2019GetafixLT,confix} techniques rely on a set of predefined templates and rules that are limited to specific software bug patterns; adding support for a new type of bug is manual and requires domain-specific knowledge in a given programming language. Instead of hard-coding error detection and repair patterns, we can automatically learn them from code examples of developer made mistakes and repairs, through  deep learning~\cite{DeepFixFC,deepdelta, dlfix,sequencer, coconut}. 

To apply learning-based techniques for software analysis, the source code needs to be vectorized. It is, however, imperative to first delineate what information in the source code  should be included as input for vectorization.  While syntactical representation of source code for vectorization has gained traction in the literature in recent years, semantic information has received less attention. In particular, the notion of \emph{context} pertaining to an erroneous statement in the code has been largely treated in an ad-hoc and arbitrary fashion. For instance, some techniques merely focus on the buggy statement~\cite{pradeloopsla, hata2019learning} and ignore context. Others use the enclosing file~\cite{hoppity,subroutineSummarization}, enclosing class~\cite{sequencer}, enclosing function~\cite{tufano:tosem:19,coconut}, or encapsulating AST subtrees~\cite{dlfix} as context, often with a hard-coded bounding limit on the number of tokens.

Arbitrarily including code as context neither captures the true semantics of the buggy statement nor encompasses essential fix-ingredients. 
For developers, context plays a significant role in understanding a bug and determining a potential fix. This is true in case of machine learning models, where too much information in the input introduces noise that can affect the repair accuracy of the model~\cite{noiseML} and too little information can lead to overfitting or relevant data loss, leading to incorrect generation of patches.
This poses questions pertaining to what is relevant context, how to collect it, what role the repair ingredients should play, and how relevant information related to both the erroneous and fixed code should be represented for deep learning consumption. 

Finding adequate context ingredients is vital to overcoming this limitation.  
In fact, when a developer tries to fix a buggy line of code, they start from the buggy line and examine all the ingredients, such as the variables and function calls used in that line. They then go backward in the code, investigating where such ingredients have been defined, used, and modified throughout the code to understand the error.  Our insight is that such relevant information can help a deep learning approach better reason about bug fixes.   In particular, we propose to adopt backward slicing analysis for extracting  contextual information in the form of code directly related to a buggy statement as well as its repaired ingredients, which we call \emph{dual slicing} in this paper.  Our approach, implemented in a tool called \toolname, extracts  dual slicing-based context from the buggy and fixed files through inter and intraprocedural control and data flow analysis, transforms the slices to AST-based graph representations, and uses a Graph Neural Network (GNN) to train a model. To evaluate our dual slicing approach, we compare against four state-of-the-art  repair techniques, and our results show that \toolname outperforms all four. 

Our work makes the following contributions: 

\begin{itemize}

	\item A technique for extracting contextual information to enhance deep learning program repair.  Our program slicing uses control and data flow analysis to find code that is relevant and applies the notion of \emph{dual slicing} to capture context from both the buggy and fixed code. It requires no hard-coded bound on the number of tokens to limit the scope of the context. 
	
	\item  An evaluation of our dual slicing technique and comparison with four state-of-the-art learning-based program repair techniques. We train models on 91,181 pairs of buggy and fixed JavaScript files.  \toolname achieves 42\% ($\frac{4,781}{11,397}$) repair accuracy within top-3 predictions, which is  between 1.5 to 3.7 times higher than existing techniques. 


	\item A quantitative analysis of the type and amount of information available for a learning model as well as a qualitative report on the type of bugs that \toolname can fix; 891 bugs are exclusively fixed by \toolname. 
	
	\item The implementation of our technique, \toolname, which is available~\cite{katana}; it includes our dataset, model and JavaScript program slicer, compatible with the latest JavaScript ES10.

\end{itemize}

%By training a model on 91,181 pairs of sliced buggy and fixed files, 

\begin{comment}
%Debugging and fixing bugs is an inevitable part of software engineering. 
According to a recent survey conducted among 1000 developers globally, about a third of them spend up to 10 hours a week fixing bugs instead of writing code. As a program becomes more complex, the probability of bugs also subsequently increasess. Different program repair techniques have been proposed in recent years to automate this process of fixing buggy programs. Traditional ways of detecting errors and repairing programs rely on a pre-defined set of rules~\cite{genprog,Scott2019GetafixLT,confix}. These techniques are somewhat limited as adding support for new types of bugs is a manual process and requires domain and programming language expertise. Deep learning-based approaches~\cite{DeepFixFC,deepdelta, dlfix,sequencer, coconut} for fixing programs have been gaining much traction lately.

Initially, deep learning-based bug detection or program repair used only the buggy line as input to generate potential fixes~\cite{pradeldeepbugsoopsla, hata2019learning}. It is challenging to devise a patch for a buggy line of code without looking into the surrounding lines, method or class. As a developer, it is hard or often impossible to write fix for a buggy piece of code without considering the context from surrounding code. To fix a bug, a developer first has to determine the location of the bug and observe the surrounding usage context to write a fix accordingly. Therefore, current repair techniques extract context considering the proximity with respect to the buggy line and with varying levels like enclosing method or class~\cite{dlfix,coconut,sequencer,tufano:tosem:19}. However, current techniques use contextual information naively without considering program analysis techniques such as data or control flow. We believe that arbitrarily treating the code surrounding the buggy or fixed statement as context neither captures the true semantics of the buggy code nor encompasses all the related information to fix a bug. In this work, we propose \toolname, which is the first to apply program slicing based context on a learning-based repair task. Program slicing is a technique used for extracting a subset of a program that is relevant to variables of interest at a given point. This technique is often used in debugging, program comprehension and maintenance. We hypothesize that by using the slice of a buggy line, the resulting subset of the code has all the relevant information needed to generate a fix. This hypothesis stems from the fact that developers tend to focus on those statements where the variables in a buggy line have been modified prior to the bug. We employ a GNN model to verify the effectiveness of \toolname in repairing a wide variety of real bugs mined from JavaScript codebases. By training the model on 91,181 pairs of sliced buggy and fixed files, \toolname can achieve 41.95\% accuracy with top-3 predictions.

The overall contribution of this paper is as follows:

\begin{itemize}
	\item A novel concept known as \emph{dual slicing} where we use the slice of both the bug and patch in buggy and fixed as context to train the model and achieve a higher accuracy of 41.95\%. This approach yielded upto 3.7 times more accuracy than the state-of-the-art context-aware program repair techniques.
	\item A quantitative analysis of the information availability for a learning model by leveraging \toolname. Additionally, we report on the type of bugs that our technique can fix.
	\item A framework, called \toolname~\cite{katana}, which includes our code, dataset, and JavaScript slicing analysis framework, compatible with the latest JavaScript ES6 and ES7 syntax.
\end{itemize}

Our findings show that \toolname is effective to reduce noise and can retain the relevant code slices surrounding the buggy line and its corresponding patch. We compared with the state-of-the-art context-aware learning-based repair models and demonstrated that our technique outperforms all of them. Dual slicing which leverages both the buggy and fixed code as context is novel to the best of our knowledge for any learning-based source code processing task. Using dual slicing, \toolname can accurately detect and fix defects in 4,781 of 11,397 programs in an end-to-end manner.
\end{comment}


==> motivating-example.tex <==
% !TEX root =  ../main.tex
\section{Motivation}
Context is essentially the background information related to a particular problem depending on the domain. The importance of context has been discussed in natural language processing tasks~\cite{contextNLP} for establishing semantic similarity between words. For a human developer, context is key in understanding and creating a fix for a buggy program. Therefore, different types of context in both machine learning and rule-based approaches have been applied for fixing a bug~\cite{capgen,dlfix, coconut, sequencer}.   In case of a program repair, the context is typically considered as the surrounding source code relevant to the buggy statement. %Therefore, this notion of context same concept has been applied to machine learning models in learning program repair. 
Current state-of-the-art learning based program repair approaches employ context in various ways and many of them use sequence-based and tree/graph based source code representation for learning program repair. These approaches use the buggy line with enclosing class \cite{sequencer}, enclosing function \cite{coconut,tufano:tosem:19}, buggy subtree \cite{dlfix}, or the whole file \cite{hoppity} for capturing the context of a buggy line. However, all these approaches have a bounding limit for processing the buggy line. The sequence-based approaches use a maximum token limit (e.g., 1,000 tokens~\cite{sequencer}), within which they extract buggy methods or classes to avoid truncated sequences. Similarly, current graph-based learning techniques use a maximum node limit (e.g., 500 nodes~\cite{hoppity}) for program repair. In practice, we cannot expect real world bugs to always be enclosed within small/medium sized methods or be limited to an arbitrary number of tokens or AST nodes. Therefore, this kind of quantitative constraint can potentially cause some important information pertaining to the bug fixes to be truncated and the overall context may even lose semantic meaning. In addition, increasing the limit on the number of tokens or nodes may add noise to the model.

\begin{lstlisting}[firstnumber=1]
'use strict';
import ENV from 'pass-ember/config/environment';
\end{lstlisting}	  
\vspace{-\baselineskip}
\begin{lstlisting}[firstnumber=3, backgroundcolor=\color{highlight}]
import { get } from '@ember/object';
import CheckSessionRoute from '../../check-session-route';
function service(user) {
	return {
		...user,
		userToken: get('currentUser.accessKey'),
		userSecret:  get('currentUser.userSecret'),
	};
}
const user = get('currentUser.user');
export default CheckSessionRoute.extend({
-   currentUser: service(),
+   currentUser: service(user),
	\end{lstlisting}
	\vspace{-\baselineskip}
	\begin{lstlisting}[firstnumber=15]
	model() {
		...
	}
	\end{lstlisting}
	\vspace{-\baselineskip}
	\begin{lstlisting}[firstnumber=30]
	...
	\end{lstlisting}
	\vspace{-\baselineskip}
	\begin{lstlisting}[firstnumber=66, backgroundcolor=\color{highlight}, label={lst:mot1}, caption={Sliced program with missing function argument},captionpos=b]
}); 
\end{lstlisting}

We will use Listing \ref{lst:mot1}, which shows a real bug and its fix for a JavaScript project on GitHub, as a running example. This type of bug is common in many languages and falls under \emph{Same function more args} pattern as categorized by Karampatsis and  Sutton~\cite{minesstubs}. Let us consider how a developer would go about fixing the bug here. After localizing the faulty line of code, they would try to determine the root cause of the bug. To do so, they would analyze how the variables or functions in the faulty line have been affected in the previous lines. The developer notices that the property \code{currentUser} is invoking a function call to \code{service}. After examining the function declaration, they notice that \code{service} expects a required \code{user} argument and that the buggy line is not passing any arguments. The developer identifies the cause of the fault and generates a fix by passing the missing argument, \code{user} declared in line 12, to the function call. 

Having too large of a context, especially if the method/class enclosing the buggy line is huge or has many dependencies can cause significant overhead~\cite{developersBugs}. 
By limiting the scope to only lines relevant to the fault, the developer can avoid information overload during the process of debugging and repairing the program.

In Listing \ref{lst:mot1}, the highlighted code indicates the portion relevant for the developer to understand and fix the bug in line 14.
The original buggy file in this example contained 66 lines of code and by focusing only on the relevant lines, the attention decreases to 13 lines. In practice, these kinds of bugs are pertinent in much more complex settings containing many lines and functions with more arguments. Furthermore, if we were to follow the approach of some of the current deep learning models, and extract only the enclosed method or enclosed class of the buggy line, then we would lose meaningful context outside the enclosing scope like the \code{user} variable and \code{service} function that were necessary for the developer in generating the correct fix. 

Our insight is that for context, instead of constraining the attention to the enclosing entities or arbitrary limitations on the number of tokens/nodes, we can constrain the code to those portions that are relevant to the bug and fix through the notion of program slicing. 



==> proposed-approach.tex <==
% !TEX root =  ../main.tex
\section{Approach}

\begin{figure*}[h]
	\centering
	\includegraphics[width=\textwidth]{images/overview.pdf}
	\caption{Overview of our approach.}
	\label{fig:overview}
\end{figure*}

We hypothesize that slicing-based context can be helpful to a machine learning model that learns patterns of bug fixes. Our technique, called \toolname, is based on static program slicing to obtain relevant context with respect to the bug and its fix. This obtained slice-based context is then represented as an AST-based graph augmented with control and data flow edges. This graph is then fed into a Graph Neural Network (GNN) for training. 
Figure \ref{fig:overview} depicts the  overview of our approach. Our overall approach consists of five main steps, namely, data collection, program slicing, graph representation, training, and inference. Next, we describe each step.

%In the program slicing phase, we collect pairs of buggy and fixed files of open-source JavaScript projects and run backward slicing on the datapoints. We refer to a pair of buggy and fixed file as a datapoint. In the training phase, we preprocess the datapoints by representing them as buggy and fixed graphs, fold the dataset, feed it to a Graph Neural Network (GNN) model, tune the model with a set of hyperparameters and train the model.  Finally, in the inference stage, the model predicts the top 3 fixes for the bug and reports the accuracy. The following sections describe the different stages of \toolname in more detail.

\subsection{Data Collection}
To collect data, we chose JavaScript as the target language. According to recent StackOverflow Developer Surveys~\cite{stackOSurvey}, JavaScript stands as the most commonly used language in the world as reported by 68.62\% of professional developers. JavaScript was initially limited to client-side code running in the web browser but has gained popularity in backend development through the emergence of the Node.js\footnote{https://nodejs.org} framework. 
\change Unlike statically typed languages such as Java or C\# where many errors can be discovered at compile time, JavaScript tends to "swallow'' errors and silently continue execution. Therefore, having a good program repair tool for a dynamically typed language such as JavaScript can help developers with a seamless coding experience.\stopchange{}

We collected pairs of buggy and fixed JavaScript files by crawling commits of open-source JavaScript repositories hosted on GitHub. We narrowed down the search by focusing on  commits containing the keywords "bug", "fix"  and "resolve". \change We collected data from 1,096 github projects. We exclude duplicates from the test dataset, as well as any data points that appear in both the test and training datasets~\cite{allamanis2019adverse}. \stopchange{}Additionally, we use heuristics to filter out commits that might be feature additions or refactorings based on the number of AST differences. To this end, we consider a difference of one AST node to be a bug, similar to existing work~\cite{hoppity}. \change We exclude minified JavaScript files since our program analysis tool cannot handle those. \stopchange{} We collected a total of 113,975 datapoints, i.e., pairs of buggy and fixed JavaScript files having one AST node difference between the pairs. 

\subsection{Static Program Slicing}
We propose to use static analysis to examine the buggy line and all the ingredients, such as the variables and function calls used in that line, and backward program slicing~ \cite{weiser}, to determine  where such ingredients have been defined, used, and modified throughout the code. We use this backward slice as context in our work, which is a subset of all statements with data or control dependencies with respect to the slicing criterion $(p,V)$, which is the set of variables $V$ at the buggy program point $p$. 

{\small
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\algnewcommand\algorithmicforeach{\textbf{foreach}}
	\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
	\begin{algorithm} \caption{Extracting Backward Sliced Context}\label{alg:backwardslice}
		\begin{algorithmic}[1]
			\Require $N$: A given line number; $file$: A given file
			\Ensure List: String: List of statements
			\State $entitySet \gets getEntities(N, file)$
			\State $contextLines \gets \{N\}$
			\ForEach {$entity \in entitySet $}
			\State \Call{BackwardSlice}{$entity$, $contextLines$}
			\EndFor
			\State \Return $getStatements(contextLines)$
			\space
			\Function{BackwardSlice}{$ent$, $contextLines$}
			\ForEach {$ref \in ent.refs() $}
			\If{$ref.ent()$ is control-dependent or data-dependent on $ent$}
			\State $N \gets ref.line()$
			\State $contextLines \gets contextLines \cup N$
			\State $entitySet \gets getEntities(N, file)$
			\ForEach {$entity \in entitySet $}
			\State \Call{BackwardSlice}{$entity$, $contextLines$}
			\EndFor
			\EndIf
			\EndFor
			\EndFunction
		\end{algorithmic}
	\end{algorithm}
}

There are two types of program slicing analysis, namely, inter-procedural and intra-procedural analysis. Intra-procedural analysis is performed within the scope of the function and inter-procedural analysis is performed within the whole program. We opted for performing both inter-procedural and intra-procedural analysis but limiting the slicing scope within the JavaScript file. The reason for such a choice is that only 12\% (13,964) of the 113,975 datapoints have the buggy line enclosed within a function and 3\% (22,940)  have the buggy line as part of a class. In 85\% (97,071), the buggy line is part of the global scope. 
In JavaScript, the global code can access all the constructs within a function, and the global code supports stepwise execution, just like functions do. This is unlike languages such as Java where the \code{main} method is required as the entry point for code execution. For this reason, we go beyond intra-procedural program analysis to capture a broad spectrum of datapoints.

We analyze each datapoint in our dataset to collect the necessary information to conduct the slicing analysis. \change In order to determine the slicing criterion, we first perform a diff analysis between the buggy and fixed lines to obtain the buggy line number. We then feed this line number to our slicing framework and extract the variables and function calls used in that line.\stopchange{} For extracting the contextual statements through static backward slicing, we incorporate both control flow and data flow analysis and identify the sliced statements where applicable. 

\change Algorithm~\autoref{alg:backwardslice} illustrates a high-level description of the steps used in extracting the context from a given line number, $N$ and $file$. Specifically, Algorithm~\autoref{alg:backwardslice} extracts the entities (i.e. variables, functions, object properties) from the given buggy or fixed line in a file. Algorithm~\autoref{alg:backwardslice} then iterates through all the entities to obtain all the $contextLines$ using backward slicing analysis. $contextLines$ is a set of line numbers of the sliced context. In the $BackwardSlice$ function, Algorithm~\autoref{alg:backwardslice} iterates through all the references in a given entity; if the referenced entity is control or data-dependent, then the corresponding line is added to $contextLines$; this process continues recursively to obtain the backward slice of the referenced entities. Finally, the algorithm constructs the source code statements from the $contextLines$ to return the output. Here, the $getStatements$ function ensures that all the closures of a given context line are extracted correctly, as it is a challenging process in a dynamic language such as JavaScript. For example, unlike Java, a semicolon is not required in JavaScript for declaration or expression statements; in such cases, we consider the new line as the end of a statement. The buggy line is within a loop or conditional statement in some cases. In such buggy statements, we determine the closure through control flow analysis to avoid an incomplete context with backward slicing. \stopchange{}

\begin{lstlisting}[label={lst:buggySliced}, caption={Sliced Buggy File},captionpos=b]
import { get } from '@ember/object';
import CheckSessionRoute from '../../check-session-route';
function service(user) {
	return {
		...user,
		userToken: get('currentUser.accessKey'),
		userSecret:  get('currentUser.userSecret'),
	};
}
export default CheckSessionRoute.extend({
-	 currentUser: service(),
});  
\end{lstlisting}

\begin{lstlisting}[label={lst:singleSliced}, caption={Single Sliced Fixed File},captionpos=b]
import { get } from '@ember/object';
import CheckSessionRoute from '../../check-session-route';
function service(user) {
	return {
		...user,
		userToken: get('currentUser.accessKey'),
		userSecret:  get('currentUser.userSecret'),
	};
}
export default CheckSessionRoute.extend({
+   currentUser: service(user),
}); 
\end{lstlisting}

Our extracted datapoints of buggy and fixed files contain the whole JavaScript code with only the bug, and the patch that contains the difference at the same buggy line. We propose two types of slicing mechanisms, namely single slicing and dual slicing. For each, we generate a separate set of datasets and conduct experiments to measure their effectiveness in repairing programs. These two types of slicing mechanisms are described below.

\header{Single Slicing}
Single slicing analysis is used for extracting context with respect to the buggy line. We start off by first taking the buggy line as the slicing criterion to capture the backward slice statements as context. This generates a buggy file with only the backward sliced statements as context. We then attach this context of the buggy file to the correct line and generate the fixed version of the buggy file. We call this \emph{single slicing} because backward slicing has been applied only on the buggy file and the context of the buggy file is simply transferred to the fixed file. Listing \ref{lst:buggySliced} and \ref{lst:singleSliced} demonstrate the snippets of single sliced pairs of buggy and fixed files from the same example shown in Listing \ref{lst:mot1}. As the slicing criterion was the buggy line, the fixed file contains the same sliced context of the buggy file and contains no information about the variable \code{user} that has been passed as a fix.

\header{Dual Slicing} 
Our intuition is that, certain repair ingredients are available in the fix context, which can  improve the overall learning process. For instance, if the fix introduces a new identifier that was not present in the buggy line, then the corresponding context will be different in the fixed version of the file. This pattern is known as \emph{Change Identifier Used}, and is commonly observed in many programming languages~\cite{minesstubs, PySStuBs}. Learning from the context of both the buggy and fixed code can provide additional semantic information to the model.  

Therefore, we hypothesize that extracting slices from both the buggy and fixed files can be more effective in conveying the contextual information to the training model. We call this notion of collecting buggy and repair contextual ingredients \emph{dual slicing}. Dual slicing analysis aims for extracting context separately from both buggy and fixed files. By using the slicing criterion from the buggy line and fixed line, we extract the sliced statements from both these lines individually to generate the sliced buggy and fixed files. Listing \ref{lst:buggySliced} and \ref{lst:dualSliced} demonstrate the dual sliced pairs of the buggy and fixed files from the motivating example of \autoref{lst:mot1}. As the slicing criteria are both the buggy and fixed lines in this approach, the fixed file contains an additional line containing the variable declaration of \code{user} in line 10 which is necessary for generating the patch as the function \code{service} expects this param.

\begin{lstlisting}[label={lst:dualSliced}, caption={Dual Sliced Fixed File},captionpos=b]
import { get } from '@ember/object';
import CheckSessionRoute from '../../check-session-route';
function service(user) {
	return {
		...user,
		userToken: get('currentUser.accessKey'),
		userSecret:  get('currentUser.userSecret'),
	};
}
const user = get('currentUser.user'); // New context
export default CheckSessionRoute.extend({
+   currentUser: service(user),
});
\end{lstlisting}

\subsection{Graph Representation}
Once we have prepared the single sliced and dual sliced datapoints, we move to the learning phase of the approach. To represent source code, we opt for graph representation. Graph representations of source code have gained popularity recently due to their ability to represent semantic information. These graphs are able to leverage the syntactic and semantic relations between the nodes via edges and to consider long-range dependencies~\cite{allamanis-represent-programs-with-graphs-2018}. 
%We generate the graph representation by  augmenting the AST with data and control-flow edges. 
For each datapoint, we create graphs for the buggy and fixed sliced files separately. We   extract the AST of each sliced files and convert it to a graph with the addition of \code{SuccToken} edges to connect leaf nodes and \code{ValueLink} edges to connect additional value nodes, following previous work~\cite{hoppity}. Figure \ref{fig:overview} illustrates the buggy and fixed graphs for the slices of our example (\autoref{lst:mot1}). After representing the source code as a graph, the resulting graphs are mapped into a vector representation using a Graph Neural Network (GNN). More specifically, given a graph $g = (V, E)$ with a set of nodes $V$ and edges $E$, we determine the $d$-dimensional representation of graph $g$ and individual node representations $\upsilon \in V$ using a function $f(g) \mapsto (\mathbb{R}^{d},\mathbb{R}^{|V| \times d})$. The node embedding is $\vec{v} = h_v^{(L)}$ where $L$ denotes the total number of propagations in the GNN via message passing \cite{gnn}. The graph representation $\vec{g}$ is the aggregation of node embeddings $h^l_v,\forall l \in 0, 1,...,L$. To aggregate $h^l_v$ for each $l$, max pooling is used, which takes the average of the $L + 1$ vectors to obtain $\vec{g}$. %~\cite{hoppity}.

\subsection{Training}
\label{subsec:training}
In this step, we split the graphs generated from the previous step into training, testing and validation using random sampling. We fold the dataset into 80\% training set, 10\% testing set, and 10\% validation set. Table \ref{table:data_split} provides the number of datapoints in the training, validation, and test datasets in our study. To train a model, we adopt a GNN architecture  %, which uses a naming agnostic approach by initializing the different node types, typically value nodes and type nodes with one-hot vectors and focus on the syntactic structure of the source code. 
that maps the graph representation into a fixed dimensional vector space. The program repair is essentially a series of graph transformation operations, from the buggy graph to the fixed graph, containing operations such as adding or deleting a node, replacing a node value or node type. \change For single slicing, the model is trained on a buggy graph, $g_{bug}$ which is the backward sliced context of only the buggy line. The output is a fixed graph, $g_{fix}$ which contains the same sliced context as $g_{bug}$, however, the buggy line is replaced with the fixed line. On the other hand, for dual slicing, the input remains the same whereas the output $g_{fix}$ contains the backward sliced context of the fixed line. \stopchange{}
%a node (\code{ADD}), deleting a node (\code{DEL}), replacing a node value (\code{REP\_VAL}), replacing a node type (\code{REP\_TYPE}) and stop (\code{NO\_OP}). The buggy and fixed files are parsed using Shift AST\footnote{https://shift-ast.org} JavaScript parser and the json diff between these files are extracted to get an array of modifications which serves as a fine-grained supervision mechanism for graph transformation. 
\begin{table}[h]
	\small
	\centering
	\caption{Dataset split for training, testing, and validation.}
	{
		\begin{tabular}{rrrr}
			\toprule
			\textbf{Train} & \textbf{Test} & \textbf{Val} & \textbf{Total} \\
			\cmidrule[0.4pt]{1-4}
			91,181 & 11,397 & 11,397 & 113,975 \\
			\bottomrule
		\end{tabular}
	}
	\label{table:data_split}
\end{table}

\header{Hyperparameter Tuning} 
Hyperparameters are important since they influence a model's overall performance. We use a batch size of 10 and tune the hyperparameters of the model for the sliced datapoints. In order to find the optimum set of hyperparameters, we use random search from a range of values in GNN layers, learning rate and dropout. We picked 2, 3 and 4 layers for the GNN model, learning rates of 0.1, 0.01, 0.001 and dropout values of 0.0, 0.1, and 0.2. We trained the model on 5 epochs with a batch size of 10 for each combination of hyperparameters. Overall, we trained 27 models during the hyperparameter search and found the best performance using 4 GNN layers, a learning rate of 0.001 and a dropout of 0.1.

\subsection{Inference}
\change After the training step, we evaluate each model using the test dataset. Given a buggy file during inference, we assume that the buggy line has already been identified in a fault localization step, similar to the current state-of-the-art learning-based repair techniques~\cite{sequencer,dlfix,coconut}. Locating the buggy line is a necessary pre-processing step to extract the backward slice as context. The model localizes the bug within the buggy graph and generates the corresponding patch. The input and output to the models during evaluation are as below: 

\begin{itemize}
	\item \emph{Training}: As described in Section~\ref{subsec:training}, we train two separate models with the single slicing and dual slicing datasets.
	\item \emph{Inference}: Input to the models remains the same during inference. For evaluating the trained single and dual sliced models, input to the model is a graph, $g_{bug}$ which is generated from the single-sliced buggy JavaScript file containing the buggy line. 
	\item \emph{Output}: For both cases, the model output is a fixed graph, $g_{fix}$, which the model tries to generate by a sequence of up to $T$ steps of transformations. We use a maximum of 20 modification steps in the graph.
\end{itemize}

\stopchange{}    
%\begin{equation}
%	p(g_{fix}|g_{bug}; \theta) = p(g_{1}|g_{bug}; \theta)p(g_{2}|g_{1}; \theta). . .p(g_{fix}|g_{T-1}; \theta)
%\end{equation}

For generating the fix for a $g_{bug}$, both single and dual slice models maintain a pool of 492 node types to predict the type; there are 5,001 values for the single slice model and 5,002 for the dual slice model, in a global value dictionary to predict node values; these types and values are extracted from our training datasets of buggy and fixed files. When generating patches to replace a node value, %\code{REP\_VAL}, 
 if a vocabulary is not in the global value dictionary, the patch is replaced with \code{UNKNOWN}. The model generates the top $k$ patches for a buggy program as a series of graph edits depending on the beam size. We consider an inferred patch as correct if the type, location and value of the fix has been accurately identified. %Finally, we evaluated the model both quantitatively and qualitatively with the same datapoints of single sliced, dual sliced and unsliced data.

\subsection{Implementation}
We implemented our technique in a tool called \toolname. Since we were not able to find any existing program slicing tool that supports the latest JavaScript ES10 features, as required for analyzing our dataset, we implemented our own JavaScript slicer for \toolname. Following previous work~\cite{capgen}, we build on top of the Understand~\cite{und} program analysis framework to analyze control flow and data flow dependencies in JavaScript code with respect to our slicing criterion. The slicer in \toolname takes as input a buggy JavaScript file, and the slicing criterion, which is the buggy line and the entities (variables, objects or functions) used in that line. It produces as output a sliced JavaScript file, which is used as context for learning repairs. The deep learning model in \toolname is based on the GNN architecture of \hoppity~\cite{hoppity}. 


==> related-work.tex <==
\section{Related Work}

\change In this section, we describe related work on (a) how slicing is used in traditional program repair, (b) the usage of contextual information in learning-based program repair, and (c) the use of slicing on different learning-based source code processing tasks.\stopchange{}

\header{Traditional Automated Program Repair} Automated program repair has received significant attention from the research community. Many APR techniques have been proposed that could be classified as search-based \cite{weimer:icse:2009, legouesNFWTSE2012, legoues:icse:2012,weimer:ase:2013, tan:relifix:icse:2015}, semantics-based \cite{nguyen:SemFix:icse:2013, ke:ase:2015}, or pattern-based \cite{liu:tbar:issta:2019, kim:icse:2013, saha-elixir-ase-1017, liu-saner-2018, liu-avatar-saner-2019, jiang-issta-2018}. From this large body of literature, CapGen~\cite{capgen} is the closest to our work, which employs program slicing for program repair. CapGen is a search-based program repair technique that leverages context based on forward and backward slicing of nodes in the AST for mutation operator selection and ingredient prioritization. However, CapGen requires domain-specific knowledge about bug and fix types, whereas our approach can learn patterns from sliced data and fix a variety of bug patterns.

\change Additionally, there are repair techniques that address specific classes of faults~\cite{luca:traditional-apr-lit-review:19}. For example,  fault specific techniques focus on repairing conditional statements~\cite{offutt:wrong-conditions:96,  xuan:wrong-conditions:17, durieux:wrong-conditions:16}, concurrency bugs~\cite{jin:concurrency-faults:11, jin:concurrency-faults:12}, string sanitization~\cite{alkhalaf:string-sanitization:14, yu:string-sanitization:11}, access control violations~\cite{son:access-control-violation:13}, or repair memory leaks~\cite{gao:memory-leaks:15}. FixMeUp~\cite{son:access-control-violation:13} targets access control violations in PHP web applications. FixMeUp applied inter-procedural program slicing on the data, and control dependence graphs to identify the statements that need to be guarded by an access control check. Instead, we applied program slicing for a learning-based model which is not bug specific.\stopchange{}

\header{Context in Learning-Based Repair} Most current learning-based repair techniques consider context in an ad-hoc manner. \hoppity~\cite{hoppity} is limited by a maximum of 500 nodes in the AST and treats the whole file as context for the buggy line. On the other hand, \sequencer~\cite{sequencer} uses the enclosing method and the class surrounding the buggy line to capture long-range dependencies between the buggy line and context. This technique is limited to 1,000 tokens, which may result in the truncation of code if the enclosing method is long, as an example. Tufano et al.~\cite{tufano:tosem:19} use buggy and fix files of small or medium-sized methods with a maximum of 50/100 tokens to learn bug fixes. They employ abstraction in the context of buggy and fixes files to mitigate the vocabulary limit. DLFix~\cite{dlfix} is a deep learning-based program repair approach that uses the context of the surrounding subtree of both the buggy line and fixed line to generate fixes using a tree-based RNN model. This context is summarized as a vector and used as weights to generate the patch for the buggy code. \coconut~\cite{coconut} uses the entire method of the buggy line as context with the buggy line and context fed as two separate inputs. \change TFix~\cite{tfix} is a learning-based system that uses a T5 model~\cite{t5-model} fine-tuned on a text-to-text patch prediction task that leverages the surrounding two lines of the buggy line as context for JavaScript errors from ESLint\footnote{https://eslint.org}. \stopchange{} All these techniques leverage context in a limited way and rely on predefined heuristics. In contrast, \toolname relies on program analysis to retrieve relevant code as context, is not bounded by predefined limits or heuristics, and leverages control and data flow information from both the buggy and fixed versions of the code. %, which can better represent repair ingredients.

\header{Slicing in Learning-Based Source Code Processing} Program slicing was explored in a learning-based vulnerability detection task~\cite{li:sysevr-vulnerability-detection:21, VulDeePeckerBinary, VulDeePeckerMulti}. VulDeePecker~\cite{VulDeePeckerBinary} trains a neural network with positive and negative examples to determine whether a code snippet suffers from vulnerability. A more recent development is µVulDeePecker~\cite{VulDeePeckerMulti},  which extends VulDeePecker to predict multiclass vulnerabilities. These techniques extract slices of the vulnerable library/API function calls and are trained on an RNN to predict vulnerabilities in code. In a recent work, Xiao et al.~\cite{slicing:apirecommendation:2021} applied program slicing to a learning-based cryptographic API Suggestion. This approach applied interprocedural backward slicing from the invocation statement of a cryptography API and trained a modified LSTM-based model for a neural-network-based API recommendation task. In \toolname, we instead (a) apply program slicing on a generative task, i.e., fix generation, (b) introduce the notion of dual slicing to learn from both the buggy and fixed-versions of the code, and (c) employ a GNN model to better capture rich structural and semantic information that is inherent to the source code instead of using RNNs that treat code as a linear stream of tokens. To the best of our knowledge, we are the first to employ slicing for learning-based program repair. 


==> threats.tex <==
\section{Threats To Validity}

\change This section describes how we addressed potential limitations that may have biased our findings. \stopchange{}

\subsection{Internal Validity} An internal threat to validity is the accurate end-to-end replication of the comparison with state of the art techniques. Two of the techniques we compared with, namely Tufano et al. ~\cite{tufano:tosem:19}, and \sequencer applied custom abstraction mechanism on the enclosing method or class of bugs in Java source code. Following Tufano et al.~\cite{tufano:tosem:19}, we implemented the same abstraction technique for JavaScript. \sequencer derives contextual information from the enclosed class of the buggy line. However, JavaScript poses unique differences from a compiled language such as, Java. As JavaScript source code is not always enclosed in a class or function, we take the entire file as the context scope in such cases to ensure that the same datapoints are preserved for a fair comparison across all techniques.

\subsection{External Validity}
We build our dataset from open source GitHub repositories of JavaScript projects. We used specific keywords to filter buggy commits following prior work~\cite{minesstubs}. One external validity is that the search heuristics used cannot ensure that all the datapoints represent actual bug fixes as some commits may contain refactoring activity or ad-hoc code changes. Nevertheless, we were able to find nine types of bug patterns pervasive across the test set, and this search criteria is consistent with other learning-based program repair studies~\cite{coconut, hoppity, tufano:tosem:19}.
 
We implemented our approach for JavaScript, and our experiments cannot conclude how effective \toolname would be for other languages. However, the fundamental challenges \toolname addresses, i.e., how to retain useful contextual information for a repair task, why context selection using a naive approach is not sufficient, how to select useful information pertaining to the buggy/fixed line, are language independent and other languages could potentially benefit from slicing-based context. \change Static program slicing requires a slicing framework for each programming language, and building such a framework is an expensive process as it requires high development cost. We therefore used a single language and built a slicing framework to evaluate our technique.

We considered a difference of one AST node for extracting buggy commits, which is similar to existing work~\cite{hoppity}. As a result, currently our approach can handle one-off errors. Existing learning-based program repair techniques~\cite{sequencer,tan:relifix:icse:2015,legouesNFWTSE2012,Scott2019GetafixLT} do not support multi-hunk changes (multiple buggy and fixed statements). However, conceptually \toolname could be extended to extract context from multiple buggy and fixed statements to better encode the repair ingredients, although this requires further evaluation in the future. In such approaches, using an ad-hoc approach would yield very large contextual information, severely limiting the effectiveness of a learning model. Therefore, we believe that fine-grained context extraction using \toolname would be even more relevant for the multi-hunk changes.\stopchange{}

%\header{Comparison with other context types} 
Some techniques do not use contextual information at all and others consider context using a different approach. For instance, Rachet~\cite{hata2019learning} only considers the buggy line without any context, whereas DLFix~\cite{dlfix} selects the buggy subtree as context. Although we did not directly compare with these in our evaluation, DLFix~\cite{dlfix}  reported to outperform Rachet, and \coconut~\cite{coconut} reported to outperform DLFix. Since \toolname is directly compared with \coconut, we can deduce, through transitive closure, that \toolname outperforms DLFix and Rachet, although direct experiments are needed to verify this empirically.

\header{Reproducibility} We have made our dataset, model, comparison framework, and \toolname's implementation available~\cite{katana} for reproducibility of the results. We further provide instructions for replicating our experimental setup.
